AutoParLLM: GNN-guided Context Generation for Zero-Shot Code Parallelization using LLMs

In-Context Learning (ICL) has been shown to be a powerful technique to augment the capabilities of LLMs for a diverse range of tasks. This work proposes \ourtool, a novel way to generate context using guidance from graph neural networks (GNNs) to generate efficient parallel codes. We evaluate \ourtool \xspace{} on $12$ applications from two well-known benchmark suites of parallel codes: NAS Parallel Benchmark and Rodinia Benchmark. Our results show that \ourtool \xspace{} improves the state-of-the-art LLMs (e.g., GPT-4) by 19.9\% in NAS and 6.48\% in Rodinia benchmark in terms of CodeBERTScore for the task of parallel code generation. Moreover, \ourtool \xspace{} improves the ability of the most powerful LLM to date, GPT-4, by achieving $\approx$17\% (on NAS benchmark) and $\approx$16\% (on Rodinia benchmark) better speedup. In addition, we propose \ourscore \xspace{} for evaluating the quality of the parallel code and show its effectiveness in evaluating parallel codes. \ourtool \xspace is available at https://github.com/quazirafi/AutoParLLM.git.

==> sections/ablation_study.tex <==
\section{Ablation Study}

In this section, we discuss the difference between the parallel versions of the loops generated using basic OMP prompt and using \ourtool \xspace{}. The generated code of GPT-3.5 and GPT-4 for Listing ~\ref{reduction-private} before and after applying the \ourtool \xspace{} guidance are shown in Figure ~\ref{fig:abl-study-1}. We can see the latter code generated with \ourtool \xspace{} is properly decorated with the "reduction" clause; however, without \ourtool \xspace{}, both LLMs fail to add the "reduction" clause. 

\lstset{basicstyle=\footnotesize\ttfamily}

% \begin{lstlisting}[label={parallel-1-regular-llm}, caption={Listing 1 parallelized by GPT-3.5 and GPT-4}, style=highlightlines]
%     ^ #pragma omp parallel for ^
%     for (i = 1; i <= 23; i += 1){
%         R23 = 0.50 * R23;  
%         T23 = 2.0 * T23; 
%     }
% \end{lstlisting}

% \begin{lstlisting}[label={parallel-1-augmented-llm}, caption={Listing 1 parallelized by GPT-3.5 and GPT-4 after applying \ourtool \xspace{} guidance}, style=highlightlines]{private}
%     ^ #pragma omp parallel for^ @reduction(*: R23, T23)@
%     for (i = 1; i <= 23; i += 1){
%           R23 = 0.50 * R23;  
%           T23 = 2.0 * T23; 
%     }
% \end{lstlisting}

\begin{figure}[h]
    \centering
    \includegraphics[width=1\linewidth]{images/abl-study-1.pdf}
    \vspace{-25pt}
    \caption{Output of GPT-3.5 and GPT-4 for Listing ~\ref{reduction-private} (a) before and, (b) after applying \ourtool \xspace guidance.}
    \vspace{-10pt}
    \label{fig:abl-study-1}
\end{figure}

% The non-parallel loop in Listing ~\ref{non-parallel}, which was wrongly classified as a parallel loop by GPT-3.5, GPT-4, and CodeGen-16B, can correctly classify the loop as non-parallel with the guidance from \ourtool. The private loop in Listing ~\ref{private} is also properly parallelized using the "private" clause by all four LLMs after \ourtool \xspace{} guidance is applied, as can be seen in Figure ~\ref{fig:abl-study-2} which also matches with the clause added by developers. All three loops in the Motivation section are successfully parallelized using our GNN-enhanced prompt-based \ourtool \xspace{} approach by mitigating the shortcomings of regular LLMs.
% \vspace{-8pt}
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=1.06\linewidth]{images/abl-study-2.pdf}
%     \vspace{-25pt}
%     \caption{Output of GPT-3.5, GPT-4 and CodeGen-16B for Listing ~\ref{private} (a) before and, (b) after applying \ourtool \xspace guidance.}
%     \label{fig:abl-study-2}
%     \vspace{-14pt}
% \end{figure}

% \begin{lstlisting}[label={parallel-2-regular-llm}, caption={Listing 3 parallelized by GPT-3.5, GPT-4, CodeLlama-34B and CodeGen-16B}, style=highlightlines]
%     ^ #pragma omp parallel for^ 
%     for (i = public.endoPoints; 
%     i <= public.allPoints-1; i += 1) {
%         private[i].point_no = i - public.endoPoints;
%         //rest of the code 
%     }
% \end{lstlisting}
% \begin{lstlisting}[caption={Listing 3 parallelized by all four LLMs after applying \ourtool guidance}, label={parallel-2-augmented-llm}, style=highlightlines]
%     ^ #pragma omp parallel for^ @ private (i) @
%     for (i = public.endoPoints; 
%     i <= public.allPoints-1; i += 1) {
%         private[i].point_no = i - public.endoPoints;
%         //rest of the code 
%     }
% \end{lstlisting}


% \begin{table}[h]
% \caption{Parallelism Discovery on autoPar Subset (Detecting parallel loops)}
% \label{autoPar-table}
% \begin{center}
% \begin{tabular}{lllll}
% \multicolumn{1}{c}{\bf Tool}  &\multicolumn{1}{c}{\bf Precision} &\multicolumn{1}{c}{\bf Recall} &\multicolumn{1}{c}{\bf F1-score} &\multicolumn{1}{c}{\bf Accuracy} 
% \\ \hline \\

% AutoPar   &    1   &   0.14   &   0.20  & 0.38 \\
% \ourtool   &     0.93    &    0.92   &   0.92   & 0.92 \\ 

% \end{tabular}
% \end{center}
% \end{table}
